RoboDepth: Robust Out-of-Distribution Depth Estimation under Corruptions

Depth estimation from monocular images is pivotal for real-world visual perception systems. While current learning-based depth estimation models train and test on meticulously curated data, they often overlook out-of-distribution (OoD) situations. Yet, in practical settings -- especially safety-critical ones like autonomous driving -- common corruptions can arise. Addressing this oversight, we introduce a comprehensive robustness test suite, RoboDepth, encompassing 18 corruptions spanning three categories: i) weather and lighting conditions; ii) sensor failures and movement; and iii) data processing anomalies. We subsequently benchmark 42 depth estimation models across indoor and outdoor scenes to assess their resilience to these corruptions. Our findings underscore that, in the absence of a dedicated robustness evaluation framework, many leading depth estimation models may be susceptible to typical corruptions. We delve into design considerations for crafting more robust depth estimation models, touching upon pre-training, augmentation, modality, model capacity, and learning paradigms. We anticipate our benchmark will establish a foundational platform for advancing robust OoD depth estimation.

==> tables/calibration.tex <==
\begin{table*}[t]
    \centering
    \caption{Depth estimation model calibration from different aspects (modality, backbone, pertaining strategy, and loss function).}
    \vspace{-0.2cm}
    \label{tab:calibration}
    \scalebox{0.66}{
    \begin{tabular}{r|c|c|c|c|c|c}
    \toprule
    \textbf{Model} & \textbf{Venue} & \textbf{Modality} & \textbf{Motivation} & \textbf{Backbone} & \textbf{Pretrain} & \textbf{Loss Function} 
    \\\midrule
    MonoDepth2 \cite{godard2019monodepth2} & ICCV'19 & Mono \& Stereo & Auto-masking \& multi-scale cues & ResNet-18/50 & ImageNet & photometric re-projection; per-pixel smoothness
    \\
    DepthHints \cite{watson2019hints} & ICCV'19 & Stereo & Complementary depth suggestions & ResNet-18 & ImageNet & photometric re-projection; per-pixel smoothness
    \\
    SC-Depth \cite{bian2019scdepth} & NeurIPS'19 & Mono & Geometry consistency constraint & ResNet-50 & CityScapes & consistency; photometric re-projection; smoothness
    \\
    CADepth \cite{yan2021cadepth} & 3DV'21 & Mono \& Stereo & Channel-wise  structural attention & ResNet-50 & ImageNet & photometric re-projection; per-pixel smoothness
    \\
    HR-Depth \cite{lyu2021hrdepth} & AAAI'21 & Mono & High-resolution features fusion & ResNet-18 & Cityscapes & photometric re-projection; per-pixel smoothness
    \\
    DIFFNet \cite{zhou2021diffnet} & BMVC'21 & Mono & Internel feature fusion mechanism & HRNet & ImageNet & photometric re-projection; per-pixel smoothness
    \\
    ManyDepth \cite{watson2021manydepth} & CVPR'21 & Multi-Mono & Sequential test-time information & ResNet-18 & ImageNet & consistency; photometric re-projection; smoothness
    \\
    FSRE-Depth \cite{jung2021fsre} & ICCV'21 & Mono & Semantics-guided triplet loss & ResNet-18 & ImageNet & semantic triplet; photometric re-projection; smoothness
    \\
    MonoViT \cite{zhao2021monovit} & 3DV'21 & Mono & Global reasoning via self-attention & MPViT & ImageNet & photometric re-projection; per-pixel smoothness
    \\
    DynaDepth \cite{zhang2022dynadepth} & ECCV'22 & Mono & Vision and IMU motion dynamics & ResNet-18/50 & ImageNet & IMU photometric; cross-sensor photometric consistency
    \\
    TriDepth \cite{chen2023tridepth} & WACV'23  & Multi-Mono & Patch-based triplet optimizing strategy & ResNet-18 & ImageNet & patch triplet; photometric re-projection; smoothness
    \\
    Lite-Mono \cite{zhang2023litemono} & CVPR'23 & Mono & Efficient mix of CNNs \& attentions & ResNet-18 & ImageNet & photometric re-projection; per-pixel smoothness
    \\\bottomrule
    \end{tabular}
    }
\end{table*}

==> tables/kitti_c_ce.tex <==
\begin{table*}[t]
\caption{The \textbf{Corruption Error (CE)} of 32 monocular depth estimation models on \textbf{\textit{KITTI-C}}. All scores are given in percentage ($\%$). Blocks from top to bottom: \textbf{[1st]} the baseline MonoDepth2$_\text{~R18}$~\cite{godard2019monodepth2}; \textbf{[2nd]} methods \textit{w/} monocular inputs; \textbf{[3rd]} methods \textit{w/} stereo inputs; \textbf{[4th]} methods \textit{w/} monocular + stereo inputs. \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-0.2cm}
\label{tab:kitti_c_ce}
\centering\scalebox{0.632}{
\begin{tabular}{r|c|cccccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mCE} & \textbf{Bright} & \textbf{Dark} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$
    \\\midrule
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $119.8$ & $140.8$ & $122.5$ & $200.7$ & $112.6$ & \cellcolor{blue!10}$78.1$ & \cellcolor{red!10}$222.5$ & \underline{$104.1$} & $95.9$ & $92.1$ & $103.0$ & $114.7$ & $109.8$ & $114.8$ & $116.2$ & $118.2$ & $116.8$ & $105.5$ & $87.2$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $106.1$ & $99.2$ & $134.3$ & $100.0$ & $97.8$ & $113.9$ & $114.4$ & \cellcolor{red!10}$161.1$ & $106.2$ & $106.5$ & $115.4$ & $95.4$ & $111.4$ & \cellcolor{blue!10}$84.9$ & $90.5$ & $93.2$ & $88.7$ & $95.2$ & $101.0$
    \\
    MonoDepth$_2$$_\text{~R50}$~\cite{godard2019monodepth2} & $113.4$ & $97.7$ & $105.0$ & $100.0$ & $103.6$ & \cellcolor{blue!10}$96.3$ & $124.6$ & \cellcolor{red!10}$175.0$ & $162.0$ & $128.2$ & $103.5$ & $100.8$ & $102.6$ & $106.5$ & $103.6$ & $108.2$ & $109.5$ & $106.9$ & $107.7$
    \\
    MaskOcc$_\text{~R18}$~\cite{schellevis2019maskocc} & $104.1$ & $100.0$ & $101.8$ & $98.7$ & $102.2$ & $96.3$ & $107.0$ & \cellcolor{red!10}$130.3$ & $121.9$ & $105.6$ & $100.0$ & $100.0$ & $95.3$ & $105.0$ & $105.4$ & $107.1$ & $107.5$ & $98.6$ & \cellcolor{blue!10}$90.3$
    \\
    DNet$_\text{~R18}$~\cite{xue2020dnet} & $104.7$ & $98.5$ & $94.3$ & $100.7$ & $114.4$ & $98.6$ & $111.8$ & \cellcolor{red!10}$142.6$ & $132.2$ & $112.0$ & $107.0$ & $101.6$ & $97.9$ & $94.3$ & $94.1$ & $95.9$ & \cellcolor{blue!10}$92.0$ & $100.0$ & $96.9$
    \\
    CADepth~\cite{yan2021cadepth} & $110.1$ & $93.1$ & $107.1$ & \cellcolor{blue!10}$91.6$ & $117.0$ & $103.5$ & $103.2$ & \cellcolor{red!10}$145.9$ & $143.4$ & $131.9$ & $103.5$ & $93.8$ & $99.5$ & $110.2$ & $111.3$ & $112.7$ & $115.5$ & $99.3$ & $99.5$
    \\
    HR-Depth~\cite{lyu2021hrdepth} & $103.7$ & $93.1$ & $103.2$ & $97.4$ & $100.7$ & $94.1$ & $113.9$ & \cellcolor{red!10}$145.9$ & $124.0$ & $121.8$ & $111.4$ & $96.1$ & $96.9$ & $94.5$ & $95.9$ & $98.8$ & $96.4$ & $\mathbf{93.1}$ & \cellcolor{blue!10}$89.8$
    \\
    DIFFNet~\cite{zhou2021diffnet} & $95.0$ & $85.4$ & $\mathbf{79.3}$ & $84.5$ & $\mathbf{71.8}$ & $68.9$ & $86.1$ & \cellcolor{red!10}$210.3$ & $136.4$ & $129.6$ & $98.0$ & $\mathbf{88.4}$ & $85.5$ & \underline{$76.0$} & \cellcolor{blue!10}\underline{$68.4$} & \underline{$75.0$} & \underline{$69.6$} & $\mathbf{93.1}$ & $103.1$
    \\
    ManyDepth$_\text{~R18}$~\cite{watson2021manydepth} & $105.4$ & $103.9$ & $97.9$ & $109.0$ & $104.0$ & $93.7$ & \cellcolor{red!10}$121.4$ & $104.1$ & $115.3$ & $97.7$ & $96.5$ & $103.9$ & $97.9$ & $112.0$ & $115.7$ & $113.8$ & $116.5$ & $101.4$ & \cellcolor{blue!10}$92.9$
    \\
    FSRE-Depth~\cite{jung2021fsre} & $99.1$ & $98.5$ & $93.2$ & $89.7$ & $85.6$ & \cellcolor{blue!10}$76.9$ & $90.9$ & $119.3$ & $112.8$ & $99.1$ & $92.0$ & $92.3$ & $92.8$ & $104.2$ & $106.4$ & $108.8$ & $104.9$ & $101.4$ & \cellcolor{red!10}$114.3$
    \\
    MonoViT~\cite{zhao2021monovit} & $79.3$ & \underline{$81.5$} & $86.8$ & \underline{$74.8$} & \underline{$76.9$} & \cellcolor{blue!10}$53.8$ & \underline{$63.6$} & $73.8$ & $84.3$ & $75.5$ & \underline{$89.1$} & $91.5$ & \underline{$75.7$} & $80.7$ & $75.3$ & $79.7$ & $74.7$ & \cellcolor{red!10}$111.7$ & $78.6$
    \\
    MonoViT$_\text{~HR}$~\cite{zhao2021monovit} & $\mathbf{75.0}$ & $78.5$ & $85.0$ & $\mathbf{73.6}$ & $81.2$ & \cellcolor{blue!10}\underline{$52.6$} & $\mathbf{62.6}$ & $\mathbf{59.4}$ & $\mathbf{70.7}$ & $\mathbf{67.1}$ & $91.5$ & $83.7$ & $\mathbf{75.1}$ & $78.7$ & $71.2$ & $76.2$ & $73.5$ & \cellcolor{red!10}$\mathbf{93.1}$ & \underline{$75.5$}
    \\
    DynaDepth$_\text{~R18}$~\cite{zhang2022dynadepth} & $110.4$ & $98.5$ & $103.2$ & $100.7$ & $104.3$ & $99.6$ & $111.2$ & \cellcolor{red!10}$205.3$ & $143.4$ & $141.2$ & $103.0$ & $98.5$ & $96.4$ & $98.7$ & $97.4$ & $98.8$ & $97.7$ & $97.2$ & \cellcolor{blue!10}$91.8$
    \\
    DynaDepth$_\text{~R50}$~\cite{zhang2022dynadepth} & $120.0$ & $98.5$ & $106.4$ & $98.1$ & $117.0$ & $107.4$ & $107.5$ & \cellcolor{red!10}$218.0$ & $187.6$ & $147.2$ & $108.5$ & \cellcolor{blue!10}$96.9$ & $102.1$ & $108.9$ & $112.3$ & $112.4$ & $115.5$ & $105.5$ & $110.2$
    \\
    RA-Depth~\cite{he2022radepth} & $112.7$ & $86.9$ & $112.1$ & $81.9$ & $86.3$ & \cellcolor{blue!10}$80.8$ & $88.2$ & \cellcolor{red!10}$204.5$ & $152.1$ & $175.0$ & $106.5$ & $94.6$ & $92.2$ & $110.2$ & $103.6$ & $118.2$ & $117.3$ & $120.7$ & $98.0$
    \\
    TriDepth$_\text{~R18}$~\cite{chen2023tridepth} & $109.3$ & $100.8$ & $107.1$ & $121.3$ & $122.0$ & $97.5$ & \cellcolor{red!10}$141.7$ & $109.8$ & $124.4$ & $98.2$ & \cellcolor{blue!10}$94.5$ & $97.7$ & $103.1$ & $108.9$ & $112.6$ & $111.8$ & $112.9$ & $97.9$ & $104.6$
    \\
    Lite-Mono$_\text{~Tiny}$~\cite{zhang2023litemono} & $92.9$ & $97.7$ & $91.8$ & $101.3$ & $81.2$ & \cellcolor{blue!10}$69.3$ & $102.1$ & \cellcolor{red!10}$105.3$ & $102.5$ & $91.7$ & $92.5$ & $98.5$ & $82.4$ & $93.2$ & $87.9$ & $98.8$ & $92.8$ & $101.4$ & $82.1$
    \\
    Lite-Mono$_\text{~Small}$~\cite{zhang2023litemono} & $100.3$ & $97.7$ & $89.6$ & $104.5$ & $90.6$ & $84.2$ & $127.3$ & \cellcolor{red!10}$144.7$ & $116.5$ & $113.9$ & $101.5$ & $99.2$ & \cellcolor{blue!10}$83.4$ & $91.2$ & $86.4$ & $93.8$ & $91.8$ & $106.2$ & $83.7$
    \\
    Lite-Mono$_\text{~Base}$~\cite{zhang2023litemono} & $93.2$ & $91.5$ & $92.5$ & $92.9$ & $88.5$ & $75.2$ & $94.7$ & $91.8$ & $97.9$ & $102.3$ & $97.5$ & $100.0$ & $90.7$ & $94.0$ & $87.4$ & $98.2$ & $93.6$ & \cellcolor{red!10}$104.1$ & \cellcolor{blue!10}$84.2$
    \\
    Lite-Mono$_\text{~Large}$~\cite{zhang2023litemono} & $90.8$ & $84.6$ & \underline{$81.1$} & $81.3$ & $92.1$ & $84.7$ & $79.7$ & $91.0$ & $93.0$ & $101.9$ & $95.5$ & $93.8$ & \cellcolor{blue!10}$76.7$ & $94.5$ & $89.5$ & $96.8$ & $93.3$ & \cellcolor{red!10}$110.3$ & $93.9$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $117.7$ & $102.3$ & $124.3$ & $103.9$ & $110.1$ & $100.8$ & $125.1$ & \cellcolor{red!10}$159.8$ & $137.2$ & $122.2$ & $104.0$ & $104.7$ & $103.6$ & $128.1$ & $130.9$ & $136.2$ & $127.1$ & $99.3$ & \cellcolor{blue!10}$99.0$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $129.0$ & $139.2$ & $150.7$ & $188.4$ & $127.1$ & \cellcolor{blue!10}$85.1$ & $182.9$ & $109.0$ & $95.9$ & $100.5$ & $113.9$ & $120.9$ & $122.3$ & $140.4$ & $145.0$ & \cellcolor{red!10}$153.2$ & $143.3$ & $113.1$ & $90.8$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $111.5$ & $101.5$ & $101.8$ & $107.7$ & $128.5$ & $103.5$ & $127.3$ & \cellcolor{red!10}$177.1$ & $128.9$ & $129.2$ & $122.4$ & $100.8$ & $106.7$ & $89.3$ & \cellcolor{blue!10}$88.2$ & $94.7$ & $88.7$ & $103.5$ & $106.6$
    \\
    DepthHints~\cite{watson2019hints} & $111.4$ & $95.4$ & $110.7$ & $88.4$ & $115.9$ & $100.8$ & \cellcolor{blue!10}$87.7$ & $143.4$ & \cellcolor{red!10}$169.4$ & $121.8$ & $97.5$ & $100.8$ & $99.5$ & $114.6$ & $114.9$ & $121.2$ & $117.3$ & $108.3$ & $98.0$
    \\
    DepthHints$_\text{~nopt}$~\cite{watson2019hints} & $141.6$ & $133.1$ & $170.0$ & $194.2$ & $135.0$ & \cellcolor{blue!10}$90.6$ & \cellcolor{red!10}$210.2$ & $146.3$ & $119.4$ & $111.6$ & $114.9$ & $110.1$ & $128.0$ & $159.6$ & $169.2$ & $176.2$ & $178.4$ & $104.8$ & $97.5$
    \\
    DepthHints$_\text{~HR}$~\cite{watson2019hints} & $112.0$ & $93.9$ & $100.7$ & \cellcolor{blue!10}$91.0$ & $114.4$ & $93.9$ & $96.3$ & \cellcolor{red!10}$188.1$ & $150.0$ & $148.2$ & $130.4$ & $91.5$ & $94.8$ & $103.4$ & $108.2$ & $111.8$ & $109.3$ & $97.2$ & $93.4$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $124.3$ & $97.7$ & $144.3$ & $96.8$ & $106.5$ & $104.9$ & $106.4$ & \cellcolor{red!10}$183.2$ & $143.0$ & $131.0$ & $101.5$ & $99.2$ & $105.2$ & $150.3$ & $155.5$ & $165.0$ & $162.1$ & \underline{$93.8$} & \cellcolor{blue!10}$91.3$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $136.3$ & $148.5$ & $164.3$ & $211.6$ & $152.0$ & $83.8$ & \cellcolor{red!10}$235.3$ & $93.4$ & $91.3$ & $100.0$ & $114.4$ & $118.6$ & $118.7$ & $148.4$ & $153.2$ & $161.5$ & $156.2$ & $111.0$ & \cellcolor{blue!10}$90.3$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $106.1$ & $99.2$ & $134.3$ & $100.0$ & $97.8$ & $113.9$ & $114.4$ & \cellcolor{red!10}$161.1$ & $106.2$ & $106.5$ & $115.4$ & $95.4$ & $111.4$ & $84.9$ & $90.5$ & $93.2$ & \cellcolor{blue!10}$88.7$ & $95.2$ & $101.0$
    \\
    CADepth~\cite{yan2021cadepth} & $118.3$ & $94.6$ & $127.5$ & \cellcolor{blue!10}$88.4$ & $112.3$ & $108.8$ & \underline{$90.4$} & $138.5$ & $170.3$ & $120.4$ & $96.0$ & $97.7$ & $96.4$ & $142.2$ & $143.7$ & $154.1$ & \cellcolor{red!10}$150.0$ & $100.0$ & $98.0$
    \\
    MonoViT~\cite{zhao2021monovit} & \underline{$75.4$} & $\mathbf{80.0}$ & $87.5$ & $78.7$ & \underline{$76.9$} & \cellcolor{blue!10}$\mathbf{42.1}$ & $70.1$ & \underline{$73.4$} & \underline{$76.0$} & \underline{$74.5$} & $\mathbf{83.6}$ & \underline{$86.8$} & $76.2$ & $\mathbf{72.1}$ & $\mathbf{66.1}$ & $\mathbf{71.2}$ & $\mathbf{67.0}$ & \cellcolor{red!10}$101.4$ & $\mathbf{73.5}$
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/kitti_c_dee2.tex <==
\begin{table*}[t]
\caption{The \textbf{Depth Estimation Error (DEE)} of 32 monocular depth estimation models on the \textbf{\textit{KITTI-C}} dataset. Blocks from top to bottom: \textbf{[1st]} the baseline MonoDepth2$_\text{~R18}$~\cite{godard2019monodepth2}; \textbf{[2nd]} methods \textit{w/} monocular inputs; \textbf{[3rd]} methods \textit{w/} stereo inputs; \textbf{[4th]} methods \textit{w/} monocular + stereo inputs. \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-.2cm}
\label{tab:kitti_c_dee2}
\centering\scalebox{.64}{
\begin{tabular}{r|c|cccccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mDEE} & \textbf{Bright} & \textbf{Dark} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.119$ & $.130$ & $.280$ & $.155$ & $.277$ & $.511$ & $.187$ & $.244$ & $.242$ & $.216$ & $.201$ & $.129$ & $.193$ & $.384$ & $.389$ & $.340$ & $.388$ & $.145$ & $.196$
    \\\midrule
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.144$ & $.183$ & $.343$ & $.311$ & $.312$ & $.399$ & $.416$ & $.254$ & $.232$ & \underline{$.199$} & $\mathbf{.207}$ & \cellcolor{blue!10}$\mathbf{.148}$ & $.212$ & $.441$ & $.452$ & $.402$ & \cellcolor{red!10}$.453$ & $\mathbf{.153}$ & $\mathbf{.171}$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $.144$ & $.129$ & $.376$ & $.155$ & $.271$ & \cellcolor{red!10}$.582$ & $.214$ & $.393$ & $.257$ & $.230$ & $.232$ & \cellcolor{blue!10}$.123$ & $.215$ & $.326$ & $.352$ & $.317$ & $.344$ & $.138$ & $.198$
    \\
    MonoDepth$_2$$_\text{~R50}$~\cite{godard2019monodepth2} & $.117$ & \cellcolor{blue!10}$.127$ & $.294$ & $.155$ & $.287$ & \cellcolor{red!10}$.492$ & $.233$ & $.427$ & $.392$ & $.277$ & $.208$ & $.130$ & $.198$ & $.409$ & $.403$ & $.368$ & $.425$ & $.155$ & $.211$
    \\
    MaskOcc$_\text{~R18}$~\cite{schellevis2019maskocc} & $.117$ & $.130$ & $.285$ & $.154$ & $.283$ & \cellcolor{red!10}$.492$ & $.200$ & $.318$ & $.295$ & $.228$ & $.201$ & \cellcolor{blue!10}$.129$ & $.184$ & $.403$ & $.410$ & $.364$ & $.417$ & $.143$ & $.177$ 
    \\
    DNet$_\text{~R18}$~\cite{xue2020dnet} & $.118$ & \cellcolor{blue!10}$.128$ & $.264$ & $.156$ & $.317$ & \cellcolor{red!10}$.504$ & $.209$ & $.348$ & $.320$ & $.242$ & $.215$ & $.131$ & $.189$ & $.362$ & $.366$ & $.326$ & $.357$ & $.145$ & $.190$
    \\
    CADepth~\cite{yan2021cadepth} & $.108$ & \cellcolor{blue!10}$.121$ & $.300$ & $.142$ & $.324$ & \cellcolor{red!10}$.529$ & $.193$ & $.356$ & $.347$ & $.285$ & $.208$ & \cellcolor{blue!10}$.121$ & $.192$ & $.423$ & $.433$ & $.383$ & $.448$ & $.144$ & $.195$
    \\
    HR-Depth~\cite{lyu2021hrdepth} & $.112$ & \cellcolor{blue!10}$.121$ & $.289$ & $.151$ & $.279$ & \cellcolor{red!10}$.481$ & $.213$ & $.356$ & $.300$ & $.263$ & $.224$ & $.124$ & $.187$ & $.363$ & $.373$ & $.336$ & $.374$ & $.135$ & $.176$
    \\
    DIFFNet~\cite{zhou2021diffnet} & $.102$ & \cellcolor{blue!10}$.111$ & $\mathbf{.222}$ & $.131$ & $\mathbf{.199}$ & $.352$ & $.161$ & \cellcolor{red!10}$.513$ & $.330$ & $.280$ & $.197$ & $.114$ & $.165$ & \underline{$.292$} & \underline{$.266$} & \underline{$.255$} & \underline{$.270$} & $.135$ & $.202$
    \\
    ManyDepth~\cite{watson2021manydepth} & $.123$ & $.135$ & $.274$ & $.169$ & $.288$ & \cellcolor{red!10}$.479$ & $.227$ & $.254$ & $.279$ & $.211$ & $.194$ & \cellcolor{blue!10}$.134$ & $.189$ & $.430$ & $.450$ & $.387$ & $.452$ & $.147$ & $.182$
    \\
    FSREDepth~\cite{jung2021fsre} & $.109$ & $.128$ & $.261$ & $.139$ & $.237$ & $.393$ & $.170$ & $.291$ & $.273$ & $.214$ & $.185$ & \cellcolor{blue!10}$.119$ & $.179$ & $.400$ & \cellcolor{red!10}$.414$ & $.370$ & $.407$ & $.147$ & $.224$
    \\
    MonoViT~\cite{zhao2021monovit} & $.099$ & \cellcolor{blue!10}$\mathbf{.106}$ & $.243$ & $\mathbf{.116}$ & $.213$ & $.275$ & $\mathbf{.119}$ & \underline{$.180$} & $.204$ & $.163$ & $.179$ & $.118$ & \underline{$.146$} & \cellcolor{red!10}$.310$ & $.293$ & $.271$ & $.290$ & $.162$ & $.154$
    \\
    MonoViT$_\text{~HR}$~\cite{zhao2021monovit} & \underline{$.094$} & \cellcolor{blue!10}\underline{$.102$} & $.238$ & \underline{$.114$} & $.225$ & \underline{$.269$} & \underline{$.117$} & $\mathbf{.145}$ & $\mathbf{.171}$ & $\mathbf{.145}$ & $.184$ & $.108$ & $.145$ & \cellcolor{red!10}$.302$ & $.277$ & $.259$ & $.285$ & $.135$ & $.148$
    \\
    DynaDepth$_\text{~R18}$~\cite{zhang2022dynadepth} & $.117$ & $.128$ & $.289$ & $.156$ & $.289$ & \cellcolor{red!10}$.509$ & $.208$ & $.501$ & $.347$ & $.305$ & $.207$ & \cellcolor{blue!10}$.127$ & $.186$ & $.379$ & $.379$ & $.336$ & $.379$ & $.141$ & $.180$
    \\
    DynaDepth$_\text{~R50}$~\cite{zhang2022dynadepth} & $.113$ & $.128$ & $.298$ & $.152$ & $.324$ & \cellcolor{red!10}$.549$ & $.201$ & $.532$ & $.454$ & $.318$ & $.218$ & \cellcolor{blue!10}$.125$ & $.197$ & $.418$ & $.437$ & $.382$ & $.448$ & $.153$ & $.216$
    \\
    RA-Depth~\cite{he2022radepth} & $.096$ & \cellcolor{blue!10}$.113$ & $.314$ & $.127$ & $.239$ & $.413$ & $.165$ & \cellcolor{red!10}$.499$ & $.368$ & $.378$ & $.214$ & $.122$ & $.178$ & $.423$ & $.403$ & $.402$ & $.455$ & $.175$ & $.192$
    \\
    TriDepth$_\text{~R18}$~\cite{chen2023tridepth} & $.117$ & $.131$ & $.300$ & $.188$ & $.338$ & \cellcolor{red!10}$.498$ & $.265$ & $.268$ & $.301$ & $.212$ & $.190$ & \cellcolor{blue!10}$.126$ & $.199$ & $.418$ & $.438$ & $.380$ & $.438$ & $.142$ & $.205$
    \\
    Lite-Mono$_\text{~Tiny}$~\cite{zhang2023litemono} & $.115$ & \cellcolor{blue!10}$.127$ & $.257$ & $.157$ & \underline{$.225$} & $.354$ & $.191$ & $.257$ & $.248$ & $.198$ & $.186$ & \cellcolor{blue!10}$.127$ & $.159$ & $.358$ & $.342$ & $.336$ & \cellcolor{red!10}$.360$ & $.147$ & $.161$
    \\
    Lite-Mono$_\text{~Small}$~\cite{zhang2023litemono} & $.115$ & \cellcolor{blue!10}$.127$ & $.251$ & $.162$ & \cellcolor{red!10}$.251$ & $.430$ & $.238$ & $.353$ & $.282$ & $.246$ & $.204$ & \underline{$.128$} & $.161$ & $.350$ & $.336$ & $.319$ & $.356$ & $.154$ & $.164$
    \\
    Lite-Mono$_\text{~Base}$~\cite{zhang2023litemono} & $.110$ & \cellcolor{blue!10}$.119$ & $.259$ & $.144$ & $.245$ & \cellcolor{red!10}$.384$ & $.177$ & $.224$ & $.237$ & $.221$ & $.196$ & $.129$ & $.175$ & $.361$ & $.340$ & $.334$ & $.363$ & $.151$ & $.165$
    \\
    Lite-Mono$_\text{~Large}$~\cite{zhang2023litemono} & $.102$ & \cellcolor{blue!10}\underline{$.110$} & \underline{$.227$} & $.126$ & $.255$ & \cellcolor{red!10}$.433$ & $.149$ & $.222$ & $.225$ & $.220$ & $.192$ & $.121$ & $\mathbf{.148}$ & $.363$ & $.348$ & $.329$ & $.362$ & $.160$ & $.184$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.123$ & \cellcolor{blue!10}$.133$ & $.348$ & $.161$ & $.305$ & \cellcolor{red!10}$.515$ & $.234$ & $.390$ & $.332$ & $.264$ & $.209$ & $.135$ & $.200$ & $.492$ & $.509$ & $.463$ & $.493$ & $.144$ & $.194$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.150$ & $.181$ & $.422$ & $.292$ & $.352$ & $.435$ & $.342$ & $.266$ & $.232$ & $.217$ & $.229$ & \cellcolor{blue!10}\underline{$.156$} & $.236$ & $.539$ & \cellcolor{red!10}$.564$ & $.521$ & $.556$ & \underline{$.164$} & \underline{$.178$}
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $.117$ & $.132$ & $.285$ & $.167$ & $.356$ & \cellcolor{red!10}$.529$ & $.238$ & $.432$ & $.312$ & $.279$ & $.246$ & \cellcolor{blue!10}$.130$ & $.206$ & $.343$ & $.343$ & $.322$ & $.344$ & $.150$ & $.209$
    \\
    DepthHints~\cite{watson2019hints} & $.113$ & \cellcolor{blue!10}$.124$ & $.310$ & $.137$ & $.321$ & \cellcolor{red!10}$.515$ & $.164$ & $.350$ & $.410$ & $.263$ & $.196$ & $.130$ & $.192$ & $.440$ & $.447$ & $.412$ & $.455$ & $.157$ & $.192$
    \\
    DepthHints$_\text{~nopt}$~\cite{watson2019hints} & $.134$ & $.173$ & $.476$ & $.301$ & $.374$ & \cellcolor{red!10}$.463$ & $.393$ & $.357$ & $.289$ & $.241$ & $.231$ & \cellcolor{blue!10}$.142$ & $.247$ & $.613$ & $.658$ & $.599$ & $.692$ & $.152$ & $.191$
    \\
    DepthHints$_\text{~HR}$~\cite{watson2019hints} & $.104$ & $.122$ & $.282$ & $.141$ & $.317$ & $.480$ & $.180$ & $.459$ & $.363$ & $.320$ & $.262$ & \cellcolor{blue!10}$.118$ & $.183$ & $.397$ & $.421$ & $.380$ & \cellcolor{red!10}$.424$ & $.141$ & $.183$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.116$ & \cellcolor{blue!10}$.127$ & $.404$ & $.150$ & $.295$ & $.536$ & $.199$ & $.447$ & $.346$ & $.283$ & $.204$ & $.128$ & $.203$ & $.577$ & $.605$ & $.561$ & \cellcolor{red!10}$.629$ & $.136$ & $.179$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.146$ & $.193$ & $.460$ & $.328$ & $.421$ & $.428$ & $.440$ & $.228$ & \underline{$.221$} & $.216$ & $.230$ & \cellcolor{blue!10}$.153$ & $.229$ & $.570$ & $.596$ & $.549$ & \cellcolor{red!10}$.606$ & $.161$ & $.177$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $.114$ & $.129$ & $.376$ & $.155$ & $.271$ & \cellcolor{red!10}$.582$ & $.214$ & $.393$ & $.257$ & $.230$ & $.232$ & \cellcolor{blue!10}$.123$ & $.215$ & \underline{$.326$} & $.352$ & \underline{$.317$} & $.344$ & $.138$ & $.198$
    \\
    CADepth~\cite{yan2021cadepth} & $.110$ & \cellcolor{blue!10}$.123$ & $.357$ & $.137$ & $.311$ & $.556$ & \underline{$.169$} & $.338$ & $.412$ & $.260$ & $.193$ & $.126$ & $.186$ & $.546$ & $.559$ & $.524$ & \cellcolor{red!10}$.582$ & $.145$ & $.192$
    \\
    MonoViT~\cite{zhao2021monovit} & $\mathbf{.098}$ & \cellcolor{blue!10}$\mathbf{.104}$ & $.245$ & $.122$ & $.213$ & $\mathbf{.215}$ & $.131$ & $.179$ & $.184$ & $.161$ & \underline{$.168$} & $.112$ & $.147$ & \cellcolor{red!10}$\mathbf{.277}$ & $\mathbf{.257}$ & $\mathbf{.242}$ & $\mathbf{.260}$ & $.147$ & $.144$
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/kitti_c_rr.tex <==
\begin{table*}[t]
\caption{The \textbf{Resilience Rate (RR)} of 32 monocular depth estimation models on \textbf{\textit{KITTI-C}}. All scores are given in percentage ($\%$). Blocks from top to bottom: \textbf{[1st]} the baseline MonoDepth2$_\text{~R18}$~\cite{godard2019monodepth2}; \textbf{[2nd]} methods \textit{w/} monocular inputs; \textbf{[3rd]} methods \textit{w/} stereo inputs; \textbf{[4th]} methods \textit{w/} monocular + stereo inputs. \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-0.2cm}
\label{tab:kitti_c_rr}
\centering\scalebox{0.639}{
\begin{tabular}{r|c|cccccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mRR} & \textbf{Bright} & \textbf{Dark} & \textbf{Fog} & \textbf{Frost} & \textbf{Snow} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $84.5$ & $98.8$ & $81.7$ & $95.9$ & $82.1$ & $55.5$ & $92.3$ & $85.8$ & $86.0$ & $89.0$ & $90.7$ & $98.9$ & $91.6$ & $69.9$ & $69.4$ & $74.9$ & $69.5$ & $97.1$ & $91.3$
    \\\midrule
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $82.5$ & $95.4$ & $76.8$ & $80.5$ & $80.4$ & $70.2$ & $68.2$ & $87.2$ & $89.7$ & \underline{$93.6$} & $\mathbf{92.6}$ & \cellcolor{blue!10}$\mathbf{99.5}$ & $92.1$ & $65.3$ & $64.0$ & $69.9$ & \cellcolor{red!10}$63.9$ & $\mathbf{99.0}$ & $\mathbf{96.9}$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $82.4$ & $98.3$ & $70.4$ & $95.4$ & $82.3$ & \cellcolor{red!10}$47.2$ & $88.7$ & $68.5$ & $83.9$ & $86.9$ & $86.7$ & \cellcolor{blue!10}$99.0$ & $88.6$ & $76.1$ & $73.1$ & $77.1$ & $74.0$ & $97.3$ & $90.5$
    \\
    MonoDepth$_2$$_\text{~R50}$~\cite{godard2019monodepth2} & $80.6$ & \cellcolor{blue!10}$98.9$ & $80.0$ & $95.7$ & $80.8$ & \cellcolor{red!10}$57.5$ & $86.9$ & $64.9$ & $68.9$ & $81.9$ & $89.7$ & $98.5$ & $90.8$ & $66.9$ & $67.6$ & $71.6$ & $65.1$ & $95.7$ & $89.4$
    \\
    MaskOcc$_\text{~R18}$~\cite{schellevis2019maskocc} & $83.0$ & $98.5$ & $81.0$ & $95.9$ & $81.2$ & \cellcolor{red!10}$57.5$ & $90.6$ & $77.2$ & $79.8$ & $87.4$ & $90.5$ & \cellcolor{blue!10}$98.6$ & $92.4$ & $67.6$ & $66.8$ & $72.0$ & $66.0$ & $97.1$ & $93.2$ 
    \\
    DNet$_\text{~R18}$~\cite{xue2020dnet} & $83.3$ & \cellcolor{blue!10}$98.9$ & $83.5$ & $95.7$ & $77.4$ & \cellcolor{red!10}$56.2$ & $89.7$ & $73.9$ & $77.1$ & $85.9$ & $89.0$ & $98.5$ & $92.0$ & $72.3$ & $71.9$ & $76.4$ & $72.9$ &  $96.9$ & $91.8$
    \\
    CADepth~\cite{yan2021cadepth} & $80.1$ & \cellcolor{blue!10}$98.5$ & $78.5$ & $96.2$ & $75.8$ & \cellcolor{red!10}$52.8$ & $90.5$ & $72.2$ & $73.2$ & $80.2$ & $88.8$ & \cellcolor{blue!10}$98.5$ & $90.6$ & $64.7$ & $63.6$ & $69.2$ & $61.9$ & $96.0$ & $90.3$
    \\
    HR-Depth~\cite{lyu2021hrdepth} & $82.9$ & \cellcolor{blue!10}$99.0$ & $80.1$ & $95.6$ & $81.2$ & \cellcolor{red!10}$58.5$ & $88.6$ & $72.5$ & $78.8$ & $83.0$ & $87.4$ & $98.7$ & $91.6$ & $71.7$ & $70.6$ & $74.8$ & $70.5$ & $97.4$ & $92.8$
    \\
    DIFFNet~\cite{zhou2021diffnet} & $85.4$ & \cellcolor{blue!10}$99.0$ & $\mathbf{86.6}$ & $96.8$ & $\mathbf{89.2}$ & $72.2$ & $93.4$ & \cellcolor{red!10}$54.2$ & $74.6$ & $80.2$ & $89.4$ & $98.7$ & $93.0$ & \underline{$78.8$} & \underline{$81.7$} & \underline{$83.0$} & \underline{$81.3$} & $96.3$ & $88.9$
    \\
    ManyDepth~\cite{watson2021manydepth} & $83.1$ & $98.6$ & $82.8$ & $94.8$ & $81.2$ & \cellcolor{red!10}$59.4$ & $88.1$ & $85.1$ & $82.2$ & $90.0$ & $91.9$ & \cellcolor{blue!10}$98.8$ & $92.5$ & $65.0$ & $62.7$ & $69.9$ & $62.5$ & $97.3$ & $93.3$
    \\
    FSREDepth~\cite{jung2021fsre} & $83.9$ & $97.9$ & $82.9$ & $96.6$ & $85.6$ & $68.1$ & $93.2$ & $79.6$ & $81.6$ & $88.2$ & $91.5$ & \cellcolor{blue!10}$98.9$ & $92.1$ & $67.3$ & \cellcolor{red!10}$65.8$ & $70.7$ & $66.6$ & $95.7$ & $87.1$
    \\
    MonoViT~\cite{zhao2021monovit} & $89.2$ & \cellcolor{blue!10}$\mathbf{99.2}$ & $84.0$ & $\mathbf{98.1}$ & $87.4$ & $80.5$ & $\mathbf{97.8}$ & \underline{$91.0$} & $88.4$ & $92.9$ & $91.1$ & $97.9$ & \underline{$94.8$} & \cellcolor{red!10}$76.6$ & $78.5$ & $80.9$ & $78.8$ & $93.0$ & $93.9$
    \\
    MonoViT$_\text{~HR}$~\cite{zhao2021monovit} & \underline{$89.7$} & \cellcolor{blue!10}\underline{$99.1$} & $84.1$ & \underline{$97.8$} & $85.5$ & \underline{$80.7$} & \underline{$97.5$} & $\mathbf{94.4}$ & $\mathbf{91.5}$ & $\mathbf{94.4}$ & $90.1$ & $98.5$ & $94.4$ & \cellcolor{red!10}$77.0$ & $79.8$ & $81.8$ & $78.9$ & $95.5$ & $94.0$
    \\
    DynaDepth$_\text{~R18}$~\cite{zhang2022dynadepth} & $81.5$ & $98.8$ & $80.5$ & $95.6$ & $80.5$ & \cellcolor{red!10}$55.6$ & $89.7$ & $56.5$ & $74.0$ & $78.7$ & $89.8$ & \cellcolor{blue!10}$98.9$ & $92.2$ & $70.3$ & $70.3$ & $75.2$ & $70.3$ & $97.3$ & $92.9$
    \\
    DynaDepth$_\text{~R50}$~\cite{zhang2022dynadepth} & $78.0$ & $98.3$ & $79.1$ & $95.6$ & $76.2$ & \cellcolor{red!10}$50.9$ & $90.1$ & $52.8$ & $61.6$ & $76.9$ & $88.2$ & \cellcolor{blue!10}$98.7$ & $90.5$ & $65.6$ & $63.5$ & $69.7$ & $62.2$ & $95.5$ & $88.4$
    \\
    RA-Depth~\cite{he2022radepth} & $78.8$ & \cellcolor{blue!10}$98.1$ & $75.9$ & $96.6$ & $84.2$ & $64.9$ & $92.4$ & \cellcolor{red!10}$55.4$ & $69.9$ & $68.8$ & $87.0$ & $97.1$ & $90.9$ & $63.8$ & $66.0$ & $66.2$ & $60.3$ & $91.3$ & $89.4$
    \\
    TriDepth$_\text{~R18}$~\cite{chen2023tridepth} & $81.6$ & $98.4$ & $79.3$ & $92.0$ & $75.0$ & \cellcolor{red!10}$56.9$ & $83.2$ & $82.9$ & $79.2$ & $89.2$ & $91.7$ & \cellcolor{blue!10}$99.0$ & $90.7$ & $65.9$ & $63.7$ & $70.2$ & $63.7$ & $97.2$ & $90.0$
    \\
    Lite-Mono$_\text{~Tiny}$~\cite{zhang2023litemono} & $86.7$ & \cellcolor{blue!10}$98.6$ & $84.0$ & $95.3$ & \underline{$87.6$} & $73.0$ & $91.4$ & $84.0$ & $85.0$ & $90.6$ & $92.0$ & \cellcolor{blue!10}$98.6$ & $95.0$ & $72.5$ & $74.4$ & $75.0$ & \cellcolor{red!10}$72.3$ & $96.4$ & $94.8$
    \\
    Lite-Mono$_\text{~Small}$~\cite{zhang2023litemono} & $84.7$ & \cellcolor{blue!10}$98.6$ & $84.6$ & $94.7$ & $84.6$ & \cellcolor{red!10}$64.4$ & $86.1$ & $73.1$ & $81.1$ & $85.2$ & $89.9$ & $98.5$ & \underline{$94.8$} & $73.5$ & $75.0$ & $77.0$ & $72.8$ & $95.6$ & $94.5$
    \\
    Lite-Mono$_\text{~Base}$~\cite{zhang2023litemono} & $86.0$ & \cellcolor{blue!10}$99.0$ & $83.3$ & $96.2$ & $84.8$ & \cellcolor{red!10}$69.2$ & $92.5$ & $87.2$ & $85.7$ & $87.5$ & $90.3$ & $97.9$ & $92.7$ & $71.8$ & $74.2$ & $74.8$ & $71.6$ & $95.4$ & $93.8$
    \\
    Lite-Mono$_\text{~Large}$~\cite{zhang2023litemono} & $85.5$ & \cellcolor{blue!10}\underline{$99.1$} & \underline{$86.1$} & $97.3$ & $83.0$ & \cellcolor{red!10}$63.1$ & $94.8$ & $86.6$ & $86.3$ & $86.9$ & $90.0$ & $97.9$ & $\mathbf{94.9}$ & $70.9$ & $72.6$ & $74.7$ & $71.1$ & $93.5$ & $90.9$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $79.1$ & \cellcolor{blue!10}$98.9$ & $74.3$ & $95.7$ & $79.3$ & \cellcolor{red!10}$55.3$ & $87.3$ & $69.6$ & $76.2$ & $83.9$ & $90.2$ & $98.6$ & $91.2$ & $57.9$ & $56.0$ & $61.2$ & $57.8$ & $97.6$ & $91.9$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $79.2$ & $96.4$ & $68.0$ & $83.3$ & $76.2$ & $66.5$ & $77.4$ & $86.4$ & $90.4$ & $92.1$ & $90.7$ & \cellcolor{blue!10}\underline{$99.3$} & $89.9$ & $54.2$ & \cellcolor{red!10}$51.3$ & $56.4$ & $52.2$ & \underline{$98.4$} & \underline{$96.7$}
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $81.6$ & $98.3$ & $81.0$ & $94.3$ & $72.9$ & \cellcolor{red!10}$53.3$ & $86.3$ & $64.3$ & $77.9$ & $81.7$ & $85.4$ & \cellcolor{blue!10}$98.5$ & $89.9$ & $74.4$ & $74.4$ & $76.8$ & $74.3$ & $96.3$ & $89.6$
    \\
    DepthHints~\cite{watson2019hints} & $80.1$ & \cellcolor{blue!10}$98.8$ & $77.8$ & $97.3$ & $76.6$ & \cellcolor{red!10}$54.7$ & $94.3$ & $73.3$ & $66.5$ & $83.1$ & $90.6$ & $98.1$ & $91.1$ & $63.1$ & $62.3$ & $66.3$ & $61.4$ & $95.0$ & $91.1$
    \\
    DepthHints$_\text{~nopt}$~\cite{watson2019hints} & $79.5$ & $98.0$ & $80.1$ & $95.9$ & $76.2$ & \cellcolor{red!10}$58.0$ & $91.5$ & $60.4$ & $71.1$ & $75.9$ & $82.4$ & \cellcolor{blue!10}$98.4$ & $91.2$ & $67.3$ & $64.6$ & $69.2$ & $64.3$ & $95.9$ & $91.2$
    \\
    DepthHints$_\text{~HR}$~\cite{watson2019hints} & $73.2$ & $95.5$ & $60.5$ & $80.7$ & $72.3$ & $62.0$ & $70.1$ & $74.3$ & $82.1$ & $87.6$ & $88.8$ & \cellcolor{blue!10}$99.1$ & $87.0$ & $44.7$ & $39.5$ & $46.3$ & \cellcolor{red!10}$35.6$ & $97.9$ & $93.4$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $75.4$ & \cellcolor{blue!10}$98.8$ & $67.4$ & $96.2$ & $79.8$ & $52.5$ & $90.6$ & $62.6$ & $74.0$ & $81.1$ & $90.1$ & $98.6$ & $90.2$ & $47.9$ & $44.7$ & $49.7$ & \cellcolor{red!10}$42.0$ & $97.7$ & $92.9$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $76.7$ & $94.5$ & $63.2$ & $78.7$ & $67.8$ & $67.0$ & $65.6$ & $90.4$ & \underline{$91.2$} & $91.8$ & $90.2$ & \cellcolor{blue!10}$99.2$ & $90.3$ & $50.4$ & $47.3$ & $52.8$ & \cellcolor{red!10}$46.1$ & $98.2$ & $96.4$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & $82.4$ & $98.3$ & $70.4$ & $95.4$ & $82.3$ & \cellcolor{red!10}$47.2$ & $88.7$ & $68.5$ & $83.9$ & $86.9$ & $86.7$ & \cellcolor{blue!10}$99.0$ & $88.6$ & \underline{$76.1$} & $73.1$ & \underline{$77.1$} & $74.0$ & $97.3$ & $90.5$
    \\
    CADepth~\cite{yan2021cadepth} & $76.7$ & \cellcolor{blue!10}$98.5$ & $72.3$ & $97.0$ & $77.4$ & $49.9$ & \underline{$93.4$} & $74.4$ & $66.1$ & $83.2$ & $90.7$ & $98.2$ & $91.5$ & $51.0$ & $49.6$ & $53.5$ & \cellcolor{red!10}$47.0$ & $96.1$ & $90.8$
    \\
    MonoViT~\cite{zhao2021monovit} & $\mathbf{90.4}$ & \cellcolor{blue!10}$\mathbf{99.2}$ & $83.6$ & $97.2$ & $87.2$ & $\mathbf{86.9}$ & $96.2$ & $90.9$ & $90.4$ & $92.9$ & \underline{$92.1$} & $98.3$ & $94.5$ & \cellcolor{red!10}$\mathbf{80.1}$ & $\mathbf{82.3}$ & $\mathbf{83.9}$ & $\mathbf{82.0}$ & $94.5$ & $94.8$
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/kitti_metrics.tex <==
\begin{table*}[t]
\caption{The reproduced scores of 32 monocular depth estimation models under the standard KITTI Eigen split. Blocks from top to bottom: \textbf{[1st]} the baseline MonoDepth2$_\text{~R18}$~\cite{godard2019monodepth2}; \textbf{[2nd]} methods \textit{w/} monocular inputs; \textbf{[3rd]} methods \textit{w/} stereo inputs; \textbf{[4th]} methods \textit{w/} monocular + stereo inputs. M+S denotes models with both monocular and stereo inputs.}
\vspace{-0.2cm}
\label{tab:kitti_metrics}
\centering\scalebox{0.64}{
\begin{tabular}{r|c|c|c|c|cccc|cccc}
    \toprule
    \textbf{Method} & \textbf{Modality} & \textbf{Backbone} & \textbf{Resolution} & \textbf{Pretrain} & \cellcolor{red!10}\textbf{Abs Rel~$\downarrow$} & \cellcolor{red!10}\textbf{Sq Rel~$\downarrow$} & \cellcolor{red!10}\textbf{RMSE~$\downarrow$} & \cellcolor{red!10}\textbf{log RMSE~$\downarrow$} & \cellcolor{blue!10}$\delta<1.25$~$\uparrow$ & \cellcolor{blue!10}$\delta<1.25^2$~$\uparrow$ & \cellcolor{blue!10}$\delta<1.25^3$~$\uparrow$
    \\\midrule\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.115$ & $0.905$	& $4.864$ & $0.193$ & $0.877$ & $0.959$ & $0.981$
    \\\midrule
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & Mono & ResNet-18 & 640 x 192 & None & $0.132$ & $1.042$ & $5.138$ & $0.210$ & $0.845$ & $0.948$ & $0.977$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & Mono & ResNet-18 & 1024 x 320 & ImageNet & $0.106$ & $0.807$ & $4.631$ & $0.193$ & $0.877$ & $0.959$ & $0.980$
    \\
    MaskOcc$_\text{~R18}$~\cite{schellevis2019maskocc} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.113$ & $0.865$ & $4.788$ & $0.191$ & $0.878$ & $0.960$ & $0.981$
    \\
    DNet$_\text{~R18}$~\cite{xue2020dnet} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.114$ & $0.867$ & $4.819$ & $0.191$ & $0.877$ & $0.960$ & $0.981$
    \\
    CADepth~\cite{yan2021cadepth} & Mono & ResNet-50 & 640 x 192 & ImageNet & $0.107$ & $0.803$ & $4.592$ & $0.183$ & $0.890$ & $0.963$ & $0.983$
    \\
    HR-Depth~\cite{lyu2021hrdepth} & Mono & ResNet-18 & 640 x 192 & Cityscapes & $0.109$ & $0.792$ & $4.632$ & $0.185$ & $0.884$ & $0.962$ & $0.983$
    \\
    DIFFNet~\cite{zhou2021diffnet} & Mono & HRNet & 640 x 192 & ImageNet & $0.102$ & $0.753$ & $4.459$ & $0.179$ & $0.897$ & $0.965$ & $0.983$
    \\
    ManyDepth$_\text{~R18}$~\cite{watson2021manydepth} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.118$ & $0.894$ & $4.765$ & $0.192$ & $0.871$ & $0.959$ & $0.982$
    \\
    FSRE-Depth~\cite{jung2021fsre} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.105$ & $0.708$ & $4.546$ & $0.182$ & $0.886$ & $0.964$ & $0.983$
    \\
    MonoViT~\cite{zhao2021monovit} & Mono & MPViT & 640 x 192 & ImageNet & $0.099$ & $0.708$ & $4.373$ & $0.175$ & $0.900$ & $0.967$ & $0.984$
    \\
    MonoViT$_\text{~HR}$~\cite{zhao2021monovit} & Mono & MPViT & 1024 x 320 & ImageNet & $0.096$ & $0.713$ & $4.292$ & $0.172$ & $0.908$ & $0.968$ & $0.984$
    \\
    DynaDepth$_\text{~R18}$~\cite{zhang2022dynadepth} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.112$ & $0.839$ & $4.848$ &  $0.192$ & $0.877$ & $0.959$ & $0.981$
    \\
    DynaDepth$_\text{~R50}$~\cite{zhang2022dynadepth} & Mono & ResNet-50 & 640 x 192 & ImageNet & $0.109$ & $0.785$ & $4.645$ & $0.188$ & $0.882$ & $0.961$ & $0.982$ 
    \\
    RA-Depth~\cite{he2022radepth} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.096$ & $0.632$ & $4.216$ & $0.171$ & $0.903$ & $0.968$ & $0.985$
    \\
    TriDepth$_\text{~R18}$~\cite{chen2023tridepth} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.112$ & $0.775$ & $4.574$ & $0.186$ & $0.878$ & $0.962$ & $0.983$
    \\
    Lite-Mono$_\text{~Tiny}$~\cite{zhang2023litemono} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.110$ & $0.841$ & $4.715$ & $0.187$ & $0.880$ & $0.960$ & $0.982$ 
    \\
    Lite-Mono$_\text{~Small}$~\cite{zhang2023litemono} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.110$ & $0.809$ & $4.677$ & $0.186$ & $0.879$ & $0.961$ & $0.982$ 
    \\
    Lite-Mono$_\text{~Base}$~\cite{zhang2023litemono} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.107$ & $0.766$ & $4.560$ & $0.183$ & $0.886$ & $0.963$ & $0.983$
    \\
    Lite-Mono$_\text{~Large}$~\cite{zhang2023litemono} & Mono & ResNet-18 & 640 x 192 & ImageNet & $0.101$ & $0.732$ & $4.459$ & $0.178$ & $0.897$ & $0.965$ & $0.983$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & Stereo & ResNet-18 & 640 x 192 & ImageNet & $0.110$ & $0.877$ & $4.967$ & $0.209$ & $0.864$ & $0.948$ & $0.975$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & Stereo & ResNet-18 & 640 x 192 & None & $0.130$ & $1.143$ & $5.482$ & $0.232$ & $0.831$ & $0.933$ & $0.968$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & Stereo & ResNet-18 & 1024 x 320 & ImageNet & $0.107$ & $0.851$ & $4.776$ & $0.202$ & $0.873$ & $0.953$ & $0.977$
    \\
    DepthHints~\cite{watson2019hints} & Stereo & ResNet-18 & 640 x 192 & ImageNet & $0.104$ & $0.791$ & $4.655$ & $0.191$ & $0.878$ & $0.959$ & $0.981$
    \\
    DepthHints$_\text{~nopt+HR}$~\cite{watson2019hints} & Stereo & ResNet-18 & 1024 x 320 & None & $0.118$ & $0.971$ & $5.099$ & $0.211$ & $0.851$ & $0.947$ & $0.976$
    \\
    DepthHints$_\text{~HR}$~\cite{watson2019hints} & Stereo & ResNet-18 & 1024 x 320 & ImageNet & $0.097$ & $0.734$ & $4.454$ & $0.187$ & $0.889$ & $0.961$ & $0.981$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & M+S & ResNet-18 & 640 x 192 & ImageNet & $0.106$ & $0.821$ & $4.752$ & $0.196$ & $0.874$ & $0.957$ & $0.979$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & M+S & ResNet-18 & 640 x 192 & None & $0.127$ & $1.027$ & $5.263$ & $0.220$ & $0.836$ & $0.943$ & $0.974$
    \\
    MonoDepth$_2$$_\text{~HR}$~\cite{godard2019monodepth2} & M+S & ResNet-18 & 1024 x 320 & ImageNet & $0.106$ & $0.807$ & $4.631$ & $0.193$ & $0.877$ & $0.959$ & $0.980$
    \\
    CADepth~\cite{yan2021cadepth} & M+S & ResNet-18 & 640 x 192 & ImageNet & $0.102$ & $0.788$ & $4.645$ & $0.192$ & $0.881$ & $0.958$ & $0.980$ 
    \\
    MonoViT~\cite{zhao2021monovit} & M+S & MPViT & 640 x 192 & ImageNet & $0.098$ & $0.683$ & $4.333$ & $0.174$ & $0.904$ & $0.967$ & $0.984$ 
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/kitti_s_dee2.tex <==
\begin{table*}[t]
\caption{The \textbf{Depth Estimation Error (DEE)} of 32 monocular depth estimation models on the \textbf{\textit{KITTI-S}} dataset. Blocks from top to bottom: \textbf{[1st]} the baseline MonoDepth2$_\text{~R18}$~\cite{godard2019monodepth2}; \textbf{[2nd]} methods \textit{w/} monocular inputs; \textbf{[3rd]} methods \textit{w/} stereo inputs; \textbf{[4th]} methods \textit{w/} monocular + stereo inputs. \textbf{Bold}: Best in col. \underline{Underline}: Second best in col.}
\vspace{-.2cm}
\label{tab:kitti_s_dee2}
\centering\scalebox{.63}{
\begin{tabular}{r|c|cccccccccccc}
    \toprule
    \textbf{Method} & \textbf{mDEE} & \textbf{Cartoon} & \textbf{Digital Art} & \textbf{Ink Paint} & \textbf{Kids' Draw} & \textbf{Murals} & \textbf{Oil Paint} & \textbf{Penciling} & \textbf{Shadow Play} & \textbf{Sketch} & \textbf{Stained Glass} & \textbf{Relief} & \textbf{Water Color}
    \\\midrule\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.365$ & $.324$ & $.434$ & $.351$ & $.259$ & $.326$ & $.328$ & $.418$ & $.388$ & $.416$ & $.566$ & $.255$ & $.317$
    \\\midrule
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.378$ & $.279$ & $.289$ & $.589$ & $.235$ & $.412$ & $.249$ & $.290$ & $.589$ & $\mathbf{.288}$ & $.596$ & $.259$ & $.464$
    \\
    MaskOcc$_\text{~R18}$~\cite{schellevis2019maskocc} & $.368$ & $.358$ & $.356$ & $.260$ & $.265$ & $.358$ & $.375$ & $.333$ & $.314$ & $.576$ & $.554$ & $.288$ & $.384$
    \\
    DNet$_\text{~R18}$~\cite{xue2020dnet} & $.400$ & $.444$ & $.381$ & $.293$ & $.280$ & $.389$ & $.336$ & $.422$ & $.290$ & $.608$ & $.553$ & $.290$ & $.516$
    \\
    CADepth~\cite{yan2021cadepth} & $.406$ & $.446$ & $.380$ & $.379$ & $.250$ & $.421$ & $.413$ & $.470$ & $.317$ & $.585$ & $.543$ & $.242$ & $.401$
    \\
    HR-Depth~\cite{lyu2021hrdepth} & $.324$ & $.318$ & $.332$ & $.238$ & $.228$ & $.299$ & $.306$ & $.337$ & $.316$ & $.388$ & $.531$ & $.265$ & $.331$
    \\
    DIFFNet~\cite{zhou2021diffnet} & $.310$ & $.227$ & $.351$ & $\mathbf{.206}$ & $.206$ & $.386$ & $.244$ & $.276$ & $.289$ & $.385$ & $.502$ & $.294$ & $.360$
    \\
    ManyDepth~\cite{watson2021manydepth} & $.323$ & $.251$ & $.373$ & \underline{$.212$} & $.205$ & $.344$ & $.300$ & $.360$ & $.343$ & $.331$ & $.553$ & $.310$ & $.300$
    \\
    FSREDepth~\cite{jung2021fsre} & $.293$ & $.275$ & $.277$ & $.294$ & $.221$ & $.310$ & $.220$ & $.270$ & $.301$ & $.318$ & $.417$ & $.261$ & $.352$
    \\
    MonoViT~\cite{zhao2021monovit} & \underline{$.238$} & \underline{$.179$} & $\mathbf{.229}$ & $.252$ & \underline{$.196$} & $.240$ & \underline{$.203$} & \underline{$.237$} & \underline{$.208$} & $.325$ & \underline{$.356$} & $\mathbf{.205}$ & $\mathbf{.221}$
    \\
    DynaDepth$_\text{~R18}$~\cite{zhang2022dynadepth} & $.371$ & $.349$ & $.358$ & $.291$ & $.264$ & $.288$ & $.293$ & $.338$ & $.363$ & $.492$ & $.534$ & $.298$ & $.585$
    \\
    DynaDepth$_\text{~R50}$~\cite{zhang2022dynadepth} & $.447$ & $.502$ & $.408$ & $.259$ & $.287$ & $.398$ & $.437$ & $.492$ & $.372$ & $.595$ & $.565$ & $.460$ & $.589$
    \\
    RA-Depth~\cite{he2022radepth} & $.365$ & $.304$ & $.335$ & $.354$ & $.262$ & $.340$ & $.310$ & $.342$ & $.425$ & $.372$ & $.476$ & $.379$ & $.475$
    \\
    TriDepth$_\text{~R18}$~\cite{chen2023tridepth} & $.379$ & $.304$ & $.403$ & $.256$ & $.217$ & $.440$ & $.352$ & $.480$ & $.318$ & $.517$ & $.573$ & $.249$ & $.436$
    \\
    Lite-Mono$_\text{~Tiny}$~\cite{zhang2023litemono} & $.280$ & $.236$ & $.310$ & $.251$ & $.221$ & $.254$ & $.283$ & $.285$ & $.232$ & $.356$ & $.446$ & $.237$ & $.252$
    \\
    Lite-Mono$_\text{~Small}$~\cite{zhang2023litemono} & $.303$ & $.210$ & $.346$ & $.218$ & $.210$ & \underline{$.224$} & $.238$ & $.374$ & $.307$ & $.445$ & $.435$ & $.295$ & $.336$
    \\
    Lite-Mono$_\text{~Base}$~\cite{zhang2023litemono} & $.288$ & $.234$ & $.313$ & $.262$ & $.218$ & $.231$ & $.241$ & $.291$ & $.240$ & $.459$ & $.476$ & $.229$ & $.264$
    \\
    Lite-Mono$_\text{~Large}$~\cite{zhang2023litemono} & $.323$ & $.208$ & $.435$ & $.249$ & $.306$ & $.348$ & $.258$ & $.363$ & $.210$ & $.458$ & $.507$ & $.263$ & $.266$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.456$ & $.382$ & $.483$ & $.329$ & $.299$ & $.499$ & $.442$ & $.449$ & $.388$ & $.584$ & $.770$ & $.363$ & $.486$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.427$ & $.351$ & $.334$ & $.587$ & $.234$ & $.440$ & $.309$ & $.357$ & $.475$ & $.316$ & $.774$ & $.305$ & $.643$
    \\\midrule
    MonoDepth$_2$$_\text{~R18}$~\cite{godard2019monodepth2} & $.414$ & $.335$ & $.444$ & $.275$ & $.267$ & $.431$ & $.402$ & $.438$ & $.367$ & $.459$ & $.809$ & $.299$ & $.438$
    \\
    MonoDepth$_2$$_\text{~nopt}$~\cite{godard2019monodepth2} & $.403$ & $.336$ & $.350$ & $.510$ & $.236$ & $.445$ & $.338$ & $.394$ & $.457$ & $.321$ & $.743$ & $.264$ & $.433$
    \\
    CADepth~\cite{yan2021cadepth} & $.401$ & $.398$ & $.446$ & $.265$ & $.260$ & $.476$ & $.423$ & $.479$ & $.250$ & $.615$ & $.552$ & $.314$ & $.336$
    \\
    MonoViT~\cite{zhao2021monovit} & $\textbf{.232}$ & $\mathbf{.173}$ & \underline{$.236$} & $.224$ & $\mathbf{.192}$ & $\mathbf{.208}$ & $\mathbf{.200}$ & $\mathbf{.226}$ & $\mathbf{.205}$ & \underline{$.315$} & $\mathbf{.338}$ & \underline{$.217$} & \underline{$.250$}
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/nyudepth2_c_ce.tex <==
\begin{table*}[t]
\caption{The \textbf{Corruption Error (CE)} of 10 monocular depth estimation models on the \textbf{\textit{NYUDepth2-C}} dataset. All scores are given in percentage ($\%$). \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-0.2cm}
\label{tab:nyudepth2_c_ce}
\centering\scalebox{0.64}{
\begin{tabular}{r|c|ccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mCE} & \textbf{Bright} & \textbf{Dark} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    AdaBins$_\text{~EB5}$~\cite{bhat2021adabins} & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$ & $100.0$
    \\\midrule
    BTS$_\text{~R50}$~\cite{lee2019big} & $122.8$ & $112.9$ & $138.7$ & $125.0$ & \cellcolor{red!10}$143.4$ & $127.2$ & $125.5$ & \cellcolor{blue!10}$96.9$ & $119.0$ & $119.2$ & $113.3$ & $136.9$ & $133.3$ & $124.7$ & \underline{$112.1$} & $113.6$
    \\
    AdaBins$_\text{~R50}$~\cite{bhat2021adabins} & $134.7$ & $135.6$ & \cellcolor{red!10}$151.0$ & $136.3$ & $144.3$ & $135.9$ & $133.2$ & \cellcolor{blue!10}$101.6$ & $133.3$ & $143.1$ & $117.4$ & $138.8$ & $136.4$ & $126.6$ & $150.0$ & $137.0$
    \\
    DPT$_\text{~ViT-B}$~\cite{ranftl2021dpt} & \underline{$83.2$} & \underline{$102.3$} & \underline{$93.8$} & \underline{$84.9$} & \underline{$65.5$} & $\mathbf{80.6}$ & \underline{$84.2$} & $\mathbf{60.4}$ & \underline{$90.9$} & \underline{$109.3$} & \cellcolor{blue!10}\underline{$51.3$} & \underline{$57.0$} & \underline{$65.0$} & \underline{$52.4$} & \cellcolor{red!10}$137.9$ & \underline{$113.0$}
    \\
    SimIPU$_\text{~nopt}$~\cite{li2022simipu} & $200.2$ & $293.9$ & $220.1$ & $211.3$ & $177.0$ & $194.7$ & $217.4$ & \cellcolor{blue!10}$112.8$ & $249.0$ & $258.9$ & $119.2$ & $125.9$ & $153.1$ & $121.3$ & \cellcolor{red!10}$302.4$ & $245.5$
    \\
    SimIPU$_\text{~ImageNet}$~\cite{li2022simipu} & $163.1$ & \cellcolor{red!10}$203.8$ & $190.7$ & $177.4$ & $160.4$ & $163.6$ & $176.1$ & \cellcolor{blue!10}$109.9$ & $200.0$ & $191.4$ & $114.1$ & $123.8$ & $140.8$ & $118.2$ & $199.2$ & $176.6$
    \\
    SimIPU$_\text{~KITTI}$~\cite{li2022simipu} & $173.8$ & $247.0$ & $192.3$ & $191.5$ & $153.2$ & $161.7$ & $182.1$ & \cellcolor{blue!10}$100.5$ & $206.5$ & $220.5$ & $110.8$ & $118.2$ & $143.5$ & $116.6$ & \cellcolor{red!10}$253.2$ & $209.1$
    \\
    SimIPU$_\text{~WaymoOpen}$~\cite{li2022simipu} & $159.5$ & \cellcolor{red!10}$203.8$ & $179.4$ & $187.7$ & $161.7$ & $158.7$ & $170.1$ & \cellcolor{blue!10}$105.5$ & $167.3$ & $190.1$ & $112.6$ & $123.3$ & $141.5$ & $119.7$ & $198.4$ & $172.1$
    \\
    DepthFormer$_\text{~SwinT-1k}$~\cite{li2022depthformer} & $106.3$ & $111.4$ & \cellcolor{red!10}$143.8$ & $110.9$ & $93.6$ & $126.2$ & $103.8$ & $78.1$ & $114.4$ & $127.2$ & \cellcolor{blue!10}$75.4$ & $85.8$ & $98.3$ & $80.3$ & $129.8$ & $116.2$
    \\
    DepthFormer$_\text{~SwinT-22k}$~\cite{li2022depthformer} & $\mathbf{63.5}$ & $\mathbf{75.0}$ & $\mathbf{77.3}$ & $\mathbf{58.0}$ & $\mathbf{54.0}$ & \cellcolor{red!10}\underline{$83.5$} & $\mathbf{64.7}$ & \underline{$61.7$} & $\mathbf{73.2}$ & $\mathbf{78.8}$ & \cellcolor{blue!10}$\mathbf{40.8}$ & $\mathbf{41.7}$ & $\mathbf{50.3}$ & $\mathbf{41.3}$ & $\mathbf{81.5}$ & $\mathbf{70.1}$
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/nyudepth2_c_dee2.tex <==
\begin{table*}[t]
\caption{The \textbf{Depth Estimation Error (DEE)} of 10 monocular depth estimation models on the \textbf{\textit{NYUDepth2-C}} dataset. \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-0.2cm}
\label{tab:nyudepth2_c_dee2}
\centering\scalebox{0.647}{
\begin{tabular}{r|c|ccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mDEE} & \textbf{Bright} & \textbf{Dark} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    AdaBins$_\text{~EB5}$~\cite{bhat2021adabins} & $.122$ & $.149$ & $.269$ & $.265$ & $.337$ & $.262$ & $.231$ & $.372$ & $.182$ & $.180$ & $.442$ & $.512$ & $.392$ & $.474$ & $.139$ & $.175$
    \\\midrule
    BTS$_\text{~R50}$~\cite{lee2019big} & $.122$ & $.149$ & $.269$ & $.265$ & $.337$ & $.262$ & $.231$ & $.372$ & $.182$ & $.180$ & $.442$ & \cellcolor{red!10}$.512$ & $.392$ & $.474$ & \cellcolor{blue!10}$.139$ & $.175$
    \\
    AdaBins$_\text{~R50}$~\cite{bhat2021adabins} & $.158$ & $.179$ & $.293$ & $.289$ & $.339$ & $.280$ & $.245$ & $.390$ & $.204$ & $.216$ & $.458$ & \cellcolor{red!10}$.519$ & $.401$ & $.481$ & \cellcolor{blue!10}$.186$ & $.211$
    \\
    DPT$_\text{~ViT-B}$~\cite{ranftl2021dpt} & $\mathbf{.136}$ & \cellcolor{blue!10}$\mathbf{.136}$ & $\mathbf{.182}$ & \underline{$.180$} & $\mathbf{.154}$ & \underline{$.166$} & $\mathbf{.155}$ & \cellcolor{red!10}$.232$ & $\mathbf{.139}$ & \underline{$.165$} & $\mathbf{.200}$ & \underline{$.213$} & $\mathbf{.191}$ & $\mathbf{.199}$ & $.171$ & $.174$
    \\
    SimIPU$_\text{~nopt}$~\cite{li2022simipu} & $.372$ & $.388$ & $.427$ & $.448$ & $.416$ & $.401$ & $.400$ & $\mathbf{.433}$ & $.381$ & $\mathbf{.391}$ & $.465$ & \cellcolor{red!10}$.471$ & $.450$ & $.461$ & \cellcolor{blue!10}$.375$ & $\mathbf{.378}$
    \\
    SimIPU$_\text{~ImageNet}$~\cite{li2022simipu} & $.244$ & $.269$ & $.370$ & $.376$ & $.377$ & $.337$ & $.324$ & $.422$ & $.306$ & $.289$ & $.445$ & \cellcolor{red!10}$.463$ & $.414$ & $.449$ & \cellcolor{blue!10}\underline{$.247$} & $.272$
    \\
    SimIPU$_\text{~KITTI}$~\cite{li2022simipu} & $.312$ & $.326$ & $.373$ & $.406$ & $.360$ & $\mathbf{.333}$ & \underline{$.335$} & \underline{$.386$} & \underline{$.316$} & $\mathbf{.333}$ & $.432$ & $.442$ & $.422$ & \cellcolor{red!10}$.443$ & \cellcolor{blue!10}$\mathbf{.314}$ & \underline{$.322$}
    \\
    SimIPU$_\text{~WaymoOpen}$~\cite{li2022simipu} & $.243$ & $.269$ & $.348$ & $.398$ & $.380$ & $.327$ & $.313$ & $.405$ & $.256$ & $.287$ & $.439$ & \cellcolor{red!10}$.461$ & $.416$ & $.455$ & \cellcolor{blue!10}\underline{$.246$} & $.265$
    \\
    DepthFormer$_\text{~SwinT-1k}$~\cite{li2022depthformer} & $.125$ & \cellcolor{blue!10}$.147$ & $.279$ & $.235$ & $.220$ & $.260$ & $.191$ & $.300$ & $.175$ & $.192$ & $.294$ & \cellcolor{red!10}$.321$ & $.289$ & $.305$ & $.161$ & $.179$
    \\
    DepthFormer$_\text{~SwinT-22k}$~\cite{li2022depthformer} & \underline{$.086$} & \cellcolor{blue!10}\underline{$.099$} & \underline{$.150$} & $\mathbf{.123}$ & \underline{$.127$} & $.172$ & $.119$ & \cellcolor{red!10}$.237$ & $.112$ & $.119$ & \underline{$.159$} & $\mathbf{.156}$ & \underline{$.148$} & \underline{$.157$} & $.101$ & $.108$
    \\\bottomrule
    \end{tabular}
}
\end{table*}


==> tables/nyudepth2_c_rr.tex <==
\begin{table*}[t]
\caption{The \textbf{Resilience Rate (RR)} of 10 monocular depth estimation models on the \textbf{\textit{NYUDepth2-C}} dataset. All scores are given in percentage ($\%$). \textbf{Bold}: Best in col. \underline{Underline}: Second best in col. {\small\colorbox{blue!10}{Blue}}: Best in row. {\small\colorbox{red!10}{Red}}: Worst in row.}
\vspace{-0.2cm}
\label{tab:nyudepth2_c_rr}
\centering\scalebox{0.64}{
\begin{tabular}{r|c|ccc|cccccc|cccccc}
    \toprule
    \textbf{Method} & \textbf{mRR} & \textbf{Bright} & \textbf{Dark} & \textbf{Contr} & \textbf{Defoc} & \textbf{Glass} & \textbf{Motio} & \textbf{Zoom} & \textbf{Elast} & \textbf{Quant} & \textbf{Gaus} & \textbf{Impul} & \textbf{Shot} & \textbf{ISO} & \textbf{Pixel} & \textbf{JPEG}
    \\\midrule\midrule
    AdaBins$_\text{~EB5}$~\cite{bhat2021adabins} & $85.8$ & $97.8$ & $90.8$ & $88.7$ & $86.2$ & $89.4$ & $91.9$ & $69.4$ & $95.4$ & $95.6$ & $68.7$ & $70.5$ & $79.5$ & $69.8$ & $98.7$ & $95.3$
    \\\midrule
    BTS$_\text{~R50}$~\cite{lee2019big} & $80.6$ & $96.9$ & $83.3$ & $83.7$ & $75.5$ & $84.1$ & $87.6$ & $71.5$ & $93.2$ & $93.4$ & $63.6$ & \cellcolor{red!10}$55.6$ & $69.3$ & $59.9$ & \cellcolor{blue!10}$98.1$ & $94.0$
    \\
    AdaBins$_\text{~R50}$~\cite{bhat2021adabins} & $81.6$ & $97.5$ & $84.0$ & $84.4$ & $78.5$ & $85.5$ & $89.7$ & $72.5$ & $94.5$ & $93.1$ & $64.4$ & \cellcolor{red!10}$57.1$ & $71.1$ & $61.6$ & \cellcolor{blue!10}$96.7$ & $93.7$
    \\
    DPT$_\text{~ViT-B}$~\cite{ranftl2021dpt} & $\mathbf{95.3}$ & \cellcolor{blue!10}$\mathbf{100.0}$ & $\mathbf{94.7}$ & \underline{$94.9$} & $\mathbf{97.9}$ & \underline{$96.5$} & $\mathbf{97.8}$ & \cellcolor{red!10}$88.9$ & $\mathbf{99.7}$ & \underline{$96.6$} & $\mathbf{92.6}$ & \underline{$91.1$} & $\mathbf{93.6}$ & $\mathbf{92.7}$ & $96.0$ & $95.6$
    \\
    SimIPU$_\text{~nopt}$~\cite{li2022simipu} & $92.5$ & $97.5$ & $91.2$ & $87.9$ & $93.0$ & $95.4$ & $95.5$ & $\mathbf{90.3}$ & $98.6$ & $\mathbf{97.0}$ & $85.2$ & \cellcolor{red!10}$84.2$ & $87.6$ & $85.8$ & \cellcolor{blue!10}$99.5$ & $\mathbf{99.0}$
    \\
    SimIPU$_\text{~ImageNet}$~\cite{li2022simipu} & $85.0$ & $96.7$ & $83.3$ & $82.5$ & $82.4$ & $87.7$ & $89.4$ & $76.5$ & $91.8$ & $94.1$ & $73.4$ & \cellcolor{red!10}$71.0$ & $77.5$ & $72.9$ & \cellcolor{blue!10}\underline{$99.6$} & $96.3$
    \\
    SimIPU$_\text{~KITTI}$~\cite{li2022simipu} & $91.6$ & $98.0$ & $91.1$ & $86.3$ & $93.0$ & $\mathbf{97.0}$ & \underline{$96.7$} & \underline{$89.2$} & \underline{$99.4$} & $\mathbf{97.0}$ & $82.6$ & $81.1$ & $84.0$ & \cellcolor{red!10}$81.0$ & \cellcolor{blue!10}$\mathbf{99.7}$ & \underline{$98.6$}
    \\
    SimIPU$_\text{~WaymoOpen}$~\cite{li2022simipu} & $85.7$ & $96.6$ & $86.1$ & $79.5$ & $81.9$ & $88.9$ & $90.8$ & $78.6$ & $98.3$ & $94.2$ & $74.1$ & \cellcolor{red!10}$71.2$ & $77.2$ & $72.0$ & \cellcolor{blue!10}\underline{$99.6$} & $97.1$
    \\
    DepthFormer$_\text{~SwinT-1k}$~\cite{li2022depthformer} & $87.3$ & \cellcolor{blue!10}$97.5$ & $82.4$ & $87.4$ & $89.1$ & $84.6$ & $92.5$ & $80.0$ & $94.3$ & $92.3$ & $80.7$ & \cellcolor{red!10}$77.6$ & $81.3$ & $79.4$ & $95.9$ & $93.8$
    \\
    DepthFormer$_\text{~SwinT-22k}$~\cite{li2022depthformer} & \underline{$94.2$} & \cellcolor{blue!10}\underline{$98.6$} & \underline{$93.0$} & $\mathbf{96.0}$ & \underline{$95.5$} & $90.6$ & $96.4$ & \cellcolor{red!10}$83.5$ & $97.2$ & $96.4$ & \underline{$92.0$} & $\mathbf{92.3}$ & \underline{$93.2$} & \underline{$92.2$} & $98.4$ & $97.6$
    \\\bottomrule
    \end{tabular}
}
\end{table*}

